Krivine Machine and Taylor Expansion in a Non-uniform Setting

The Krivine machine is an abstract machine implementing the linear head reduction of lambda-calculus. Ehrhard and Regnier gave a resource sensitive version returning the annotated form of a lambda-term accounting for the resources used by the linear head reduction. These annotations take the form of terms in the resource lambda-calculus. We generalize this resource-driven Krivine machine to the case of the algebraic lambda-calculus. The latter is an extension of the pure lambda-calculus allowing for the linear combination of lambda-terms with coefficients taken from a semiring. Our machine associates a lambda-term M and a resource annotation t with a scalar k in the semiring describing some quantitative properties of the linear head reduction of M. In the particular case of non-negative real numbers and of algebraic terms M representing probability distributions, the coefficient k gives the probability that the linear head reduction actually uses exactly the resources annotated by t. In the general case, we prove that the coefficient k can be recovered from the coefficient of t in the Taylor expansion of M and from the normal form of t.

==> eptcsdata.tex <==
\providecommand{\firstpage}{24}
\providecommand{\publicationstatus}{I. Cervesato and M. Fern\'andez (Eds): Fourth International Workshop\\ on Linearity 2016 (LINEARITY'16)\\
EPTCS 238, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.238.3}{10.4204/EPTCS.238.3}}

